A Probabilistic Model of Cardiac Physiology and Electrocardiograms

An electrocardiogram (EKG) is a common, non-invasive test that measures the electrical activity of a patient's heart. EKGs contain useful diagnostic information about patient health that may be absent from other electronic health record (EHR) data. As multi-dimensional waveforms, they could be modeled using generic machine learning tools, such as a linear factor model or a variational autoencoder. We take a different approach:~we specify a model that directly represents the underlying electrophysiology of the heart and the EKG measurement process. We apply our model to two datasets, including a sample of emergency department EKG reports with missing data. We show that our model can more accurately reconstruct missing data (measured by test reconstruction error) than a standard baseline when there is significant missing data. More broadly, this physiological representation of heart function may be useful in a variety of settings, including prediction, causal analysis, and discovery.

==> figs/output-ed/rmse-table.tex <==
\begin{tabular}{lll}
\toprule
{} &            median rmse &                 mean rmse \\
model &                        &                           \\
\midrule
dip   &  \textbf{0.109 [0.093 - 0.122]} &    \textbf{0.215 [0.164 - 0.278]} \\
pca-3 &  0.183 [0.149 - 0.233] &     2.868 [0.378 - 7.486] \\
pca-6 &  0.328 [0.269 - 0.378] &  64.574 [9.066 - 155.060] \\
\bottomrule
\end{tabular}


==> figs/rmse-table.tex <==
\begin{tabular}{llll}
\toprule
model &                    dip &                  pca-3 &                  pca-6 \\
\midrule
ed  &  0.111 [0.102 - 0.119] &  0.194 [0.180 - 0.212] &  0.300 [0.281 - 0.329] \\
ptb &  0.066 [0.059 - 0.074] &  0.063 [0.059 - 0.067] &  0.058 [0.051 - 0.066] \\
\bottomrule
\end{tabular}

